"The Whole Is Greater Than the Sum of Its Parts": Optimization in Collaborative Crowdsourcing

In this work, we initiate the investigation of optimization opportunities in collaborative crowdsourcing. Many popular applications, such as collaborative document editing, sentence translation, or citizen science resort to this special form of human-based computing, where, crowd workers with appropriate skills and expertise are required to form groups to solve complex tasks. Central to any collaborative crowdsourcing process is the aspect of successful collaboration among the workers, which, for the first time, is formalized and then optimized in this work. Our formalism considers two main collaboration-related human factors, affinity and upper critical mass, appropriately adapted from organizational science and social theories. Our contributions are (a) proposing a comprehensive model for collaborative crowdsourcing optimization, (b) rigorous theoretical analyses to understand the hardness of the proposed problems, (c) an array of efficient exact and approximation algorithms with provable theoretical guarantees. Finally, we present a detailed set of experimental results stemming from two real-world collaborative crowdsourcing application us- ing Amazon Mechanical Turk, as well as conduct synthetic data analyses on scalability and qualitative aspects of our proposed algorithms. Our experimental results successfully demonstrate the efficacy of our proposed solutions.

==> algo2.tex <==
\section{Solution: Inter-Affinity-Group-Factor}
\label{sec:algo3}

\subsection{Approximation Algorithm}

\subsection{Integer Programming}


==> algorithm.tex <==
\section{Solution of the Original Problem}
\label{sec:algo1}

\textbf{IP Formulation:}
Minimize $v_t$, such that
\begin{equation}
  v_t =
  \begin{cases}
    W_1 \times A_{intra}\\ 
    + W_2 \times A_{inter}  
   \end{cases}
\end{equation}

\begin{align*} 
 q_{t} = \sum_{g=1}^{g=x_g}\sum_{u=1}^{u=|U|}s_u \times x_{ug} \geq Q_t 
\\ \sum_{g=1}^{g=x_g}\sum_{u=1}^{u=|U|}w_u  \times x_{ug} \leq C_t 
\\A_{intra} = \sum_{g=1}^{g=x_g} \sum_{\forall u,u' \in U} y_{uu'g} \times dis(u,u')
\\\sum_{g=1}^{g=x_g} \sum_{\forall u,u' \in U}y_{uu'g} \geq (x_{ug} + x_{u'g} -1)
\\A_{inter} = \sum_{i=1}^{i=x_g-1} \sum_{j=i+1}^{j=x_g} \sum_{\forall u,u' \in U} z_{uu'ij}\times dis(u,u')
\\\sum_{i=1}^{i=x_g-1} \sum_{j=i+1}^{j=x_g} \sum_{\forall u,u' \in U} z_{uu'ij} \geq (x_{ui} + x_{u'j} -1)
\\ \sum_{g=1}^{g=x_g}x_{ug}=1  \forall u \in {U}
\\\sum_{u=1}^{U}x_{ug} \leq k_t \forall g \in {G}
\\x_{ug},y_{uu'g} \in {0,1}\text{,}x_g \in \mathbb{N} 
\\W_1 + W_2=1 
\end{align*} 
 


For the first term in $v_t$ we are maximizing the skill requirement, and for the 2nd term we are minimizing the intra group dissimilarity. $x_g$ itself is a decision variable which outputs the number of groups.



Here we describe the solution for the problems mentioned before. We will show that each variant of the problem is NP-Hard. We give an approximation algorithm for the problems if there 




==> algorithm2.tex <==
\section{Solution: Intra-Affinity-Ind-Factor}
\label{sec:algo2}

%\subsubsection{Problem-1: Minimize Inter Group Sum of Distances and Intra Group Sum of Distances with Skill,Cost and Critical Mass }
%\begin{theorem}
%  Problem-1  is NP-Hard.
%\end{theorem}
%\begin{proof}
%  \begin{itemize}
%   \item Even simpler version of this problem is NP-Hard.
%  \end{itemize}
%\end{proof}

\subsection{Solution : {\tt Min-Sum,Skill,Cost}}
%\begin{theorem}
%  Problem-2  is NP-Hard.
%\end{theorem}
%\begin{proof}
%  \begin{itemize}
%   \item Even simpler version of this problem is NP-Hard.
%  \end{itemize}
%\end{proof}


Here we are giving the IP formulation of the problem


\subsection{Solution : {\tt Min-Dia,Skill,Cost}}


{\bf Approaximation Algorithm:} {\tt Min-Dia,Skill,Cost} is NP-Hard, we proposed an approximation algorithm with proven approximation guarantee. First, we call the Generic Algorithm \ref{alg_gen}. The algorithm calls another subroutine, Algorithm \ref{alg_sub_MinDia_Skill_Cost} with a parameter $\alpha$,to see if there exist a set of vertices whose maximum distance is at most twice of $\alpha$ but satisfy the skill and cost threshold. This algorithm returns a set of vertices form minimum such $\alpha$. Since cost of each worker is 1, So we select number of workers equal to the cost threshold. 

%{\bf Approaximation Algorithm} Since (Min-Diam,Skill) is NP-Hard, we proposed an approximation algorithm with proven approximation guarantee. First, we call the Generic Algorithm \ref{alg_gen}. The algorithm calls another subroutine, Algorithm \ref{alg_sub_MinDia_Skill} with a parameter $\alpha$,to see if there exist a set of vertices whose maximum distance is at most twice of $\alpha$ but satisfy the skill threshold. This algorithm returns a set of vertices form minimum such $\alpha$ which satisfy the skill threshold. 

%
\begin{algorithm}[t]
\caption{(Generic Algorithm)}
\label{alg:gen}
\begin{algorithmic}[1]
\begin{small}
\REQUIRE A set of workers (and their skill) and between every pair of workers $u,u'$, $dist(u,u')$ and the skill requirement (let us assume a single skill for now of the task $Q$\\
\STATE Sort the dissimilarities in increasing order and create an array $D$ with the sorted value.
\STATE Do a Bianry Search over $D$ to find out the smallest diameter $\alpha$ such that, $Call(Diam)$ returns success.
\IF{text{No such $\alpha$ found}}
\STATE Stop
\ENDIF

\RETURN Set of Workers returned by the $Diam$


% \STATE $i=0$
% \WHILE{the entire $D$ array is not searched} 
% \STATE $\alpha = D[i]$; 
% \STATE{$Call(Diam(\alpha,Q))$} 
% \IF{text{it returns success}} 
% \STATE{stop} 
% \RETURN results of the subroutine
% \ENDIF
% \STATE $i=i+1$
% \ENDWHILE
\end{small}
\end{algorithmic}
\end{algorithm}
%%
%\begin{algorithm}[t]
%\caption{Subroutine (Min-Diam,Skill) $Diam(d,Q)$}
%\label{alg_sub_MinDia_Skill}
%\begin{algorithmic}[1]
%\begin{small}
%\REQUIRE Takes a distance value and a skill threshold as input, uses the skill of the given set of workers, and outputs a subset of workers. It returns Success or Failure based on certain condition.
%\STATE $\mathcal{U} = \{u_1,u_2,\ldots,u_n\}$ 
%\STATE $\mathcal{V} = \{ \}$
%\STATE $i=0$
%\WHILE{$i < n$} 
%\STATE $\mathcal{V} = \{u_i\}$
%\STATE for $u' \neq u_i$
%\IF{$dis(u_i,u') \leq d$} 
%\STATE{$\mathcal{V} = \mathcal{V} \cup u'$} 
%\ENDIF
%\STATE end 
%\IF{$\Sigma_{\forall j \in \mathcal{V}} s(j) \geq Q$}
%
%\STATE return success to the main function
%\ENDIF
%\ENDWHILE
%\STATE return failure to the main function
%\end{small}
%\end{algorithmic}
%\end{algorithm}
%
%\begin{theorem}
%Algorithm~\ref{diam} has a 2-approximation factor
%\end{theorem}
%
%\begin{proof} 
%(sketch)
%\begin{itemize}
%\item Algorithm~\ref{diam} returns the first success for the smallest distance value $\alpha$. Therefore, there is no $\alpha' < \alpha$ which satisfies the skill lowerbound.
%\item A clique (set of workers) returned as Success by subroutine $Diam(\alpha,Q)$ can have the maximum distance as $2 \times \alpha$, as the workers distance satisfy triangle inequality.
%\item If there is another clique which has the diameter $\alpha$, the algorithm may choose the former over the latter. Hence the $2$-approximation. 
%\end{itemize}
%\end{proof}
%
%\textbf{Time Complexity:} The worst case complexity of Algorithm~\ref{diam} is $O(n^2logn)$.


% \begin{figure}[h]
% \centering
% \includegraphics[width=3.5in]{figures/example.pdf}
% \caption{\label{fig:ex} An example to use}
% \end{figure}

%\subsubsection{Minimize Maximum  Distance Under Quality Threshold (Min-Diameter,Skill,Cost)}
%\begin{theorem}
%  (Min-Diam,Skill,Cost) is NP-Hard.
%\end{theorem}
%\begin{proof}
%\label{prf:Min-Diam_skill}
%  \begin{itemize}
%    \item This directly follows from the previous proof.
%    \item In this case we will set each worker's cost as 1 and if there is a clique of size K then then both cost and quality threshold are satisfied with if they are set to K. 
%    
% \end{itemize}
%\end{proof}



\subsubsection{Algorithm for finding a set of workers satisfying skill thresholds}
\begin{algorithm}[t]
\caption{Subroutine (Min-Diam,Skill) $Diam(d,Q,C)$}
\label{alg_sub_MinDia_Skill_Cost}
\begin{algorithmic}[1]
\begin{small}
\REQUIRE Takes a distance value,a skill threshold and Cost threshold as input, uses the skill of the given set of workers, and outputs a subset of workers. It returns Success or Failure based on certain condition.
\STATE $\mathcal{U} = \{u_1,u_2,\ldots,u_n\}$ 
\STATE $\mathcal{V} = \{ \}$
\STATE $i=0$
\WHILE{$i < n$} 
\STATE $\mathcal{V} = \{u_i\}$
%\STATE for $u' \neq u_i$
% \IF{$dis(u_i,u') \leq d$} 
% \STATE{$\mathcal{V} = \mathcal{V} \cup u'$} 
% \ENDIF
%\STATE 
\STATE $Cand = \{x | dis(u_i,x) \leq d, x \in U\}$
\IF{$|Cand| < C -1 $}
  \STATE Return failure to the main function. 
\ELSE
  \STATE $Cand$ = {Select C-1 nodes from $Cand$ in decreasing order of their distance from $u_i$ 
  }
  \STATE $\mathcal{V} = \mathcal{V} \cup Cand$
  \IF{$\Sigma_{\forall j \in \mathcal{V}} s(j) \geq Q$}
    \STATE return success to the main function
    \ENDIF
\ENDIF
\ENDWHILE
\STATE return failure to the main fucntion.
\end{small}
\end{algorithmic}
\end{algorithm}


\subsubsection{Algorithm for satisfying a cost threshold for constant number of costs}


\subsubsection{Approximation Factor}
\begin{theorem}
(Min-Diam,Skill,Cost) has has a 2-approximation factor for the algorithm \ref{alg_sub_MinDia_Skill_Cost}.
\end{theorem}
\begin{proof} 
(sketch)
\begin{itemize}
\item Algorithm~\ref{diam} returns the first success for the smallest distance value $\alpha$. Therefore, there is no $\alpha' < \alpha$ which satisfies the skill lowerbound and cost lowerbound. 
\item A clique (set of workers) returned as Success by subroutine $Diam(\alpha,Q)$ can have the maximum distance as $2 \times \alpha$, as the workers distance satisfy triangle inequality.
\item If there is another clique which has the diameter $\alpha$, the algorithm may choose the former over the latter. Hence the $2$-approximation. 
\end{itemize}
\end{proof}

\subsubsection{Time Complexity} The worst case complexity of Algorithm~\ref{diam} is $O(n^2logn)$.



==> discussion.tex <==
\section{discussion}

[Notes]

The quality of collaboration and interaction between the workers is important(and not only the quality of the final document) because in KI-C you want recurrent workers , so motivation is important. In other words, the quality of collaboration is important because you want people to like it, to be motivated to come back, because of the cost (money spent) to profile them and because KI-C workers are not infinite/replaceable like the normal crowdsourcing ones. 
